Revisiting, Benchmarking and Exploring API Recommendation: How Far Are We?

Application Programming Interfaces (APIs), which encapsulate the implementation of specific functions as interfaces, greatly improve the efficiency of modern software development. As numbers of APIs spring up nowadays, developers can hardly be familiar with all the APIs, and usually need to search for appropriate APIs for usage. So lots of efforts have been devoted to improving the API recommendation task. However, it has been increasingly difficult to gauge the performance of new models due to the lack of a uniform definition of the task and a standardized benchmark. For example, some studies regard the task as a code completion problem; while others recommend relative APIs given natural language queries. To reduce the challenges and better facilitate future research, in this paper, we revisit the API recommendation task and aim at benchmarking the approaches. Specifically, the paper groups the approaches into two categories according to the task definition, i.e., query-based API recommendation and code-based API recommendation. We study 11 recently-proposed approaches along with 4 widely-used IDEs. One benchmark named as APIBench is then built for the two respective categories of approaches. Based on APIBench, we distill some actionable insights and challenges for API recommendation. We also achieve some implications and directions for improving the performance of recommending APIs, including data source selection, appropriate query reformulation, low resource setting, and cross-domain adaptation.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> table/javadomainres.tex <==
\begin{table*}[t]
    \centering
    \caption{The cross-domain Success Rate@10 of Java code-based API recommendation baselines. The rows list the domains where three baselines are trained and the columns list the domains where three baselines are evaluated.}
    \begin{tabular}{cccccccccccc}
    \toprule
       \multirow{2}*{\textbf{Training Domain}} & & \multicolumn{4}{c}{\textbf{PAM-MAX}} & & \multicolumn{4}{c}{\textbf{FOCUS}} \\
       \cmidrule{3-6}
       \cmidrule{8-11}
         & & Android & ML & Testing & Security & & Android & ML & Testing & Security \\
         \midrule
         Android & & \textcolor{red}{\textbf{0.43}} & 0.33 & 0.32 & 0.33 & & 0.05 & \textcolor{red}{\textbf{0.07}} & 0.06 & 0.05\\
         \specialrule{0em}{1pt}{1pt}
         ML & & 0.14 & 0.19 & \textcolor{red}{\textbf{0.21}} & 0.20 & & 0.05 & \textcolor{red}{\textbf{0.08}} & 0.07 & 0.04 \\
         \specialrule{0em}{1pt}{1pt}
         Testing & & 0.06 & \textcolor{red}{\textbf{0.15}} & 0.13 & 0.14 & & 0.05 & \textcolor{red}{\textbf{0.07}} & 0.05 & 0.05 \\
         \specialrule{0em}{1pt}{1pt}
         Security & & 0.14 & \textcolor{red}{\textbf{0.18}} & 0.14 & 0.16 & & 0.05 & 0.06 & \textcolor{red}{\textbf{0.07}} & 0.05\\
         \midrule
         General && \g 0.54 & \g 0.49 & \g 0.53 & \g 0.50 & & \g 0.06 & \g 0.15 & \g 0.16 & \g 0.09\\
         \bottomrule
    \end{tabular}
    \label{tab:javadomainres}
\end{table*}

==> table/reformex.tex <==
\begin{table*}[t]
    \centering
    \caption{Some Examples of Different Query Reformulation techniques. The highlighted words are modified/expanded by reformulation techniques. }
    \begin{tabular}{lcl}
    \toprule
        \textbf{Approach} & \textbf{Method} & \textbf{Query}  \\
    \midrule
        \multirow{2}*{NLP2API} & \multirow{2}*{expansion} & \textbf{Original:} Returns a new Document instance\\
        & & \textbf{Reformulated:} \textcolor{red}{DocumentBuilderFactory} Returns a new Document instance \\
        \midrule
        \multirow{2}*{RACK} & \multirow{2}*{expansion} & \textbf{Original:} Determine Java version through JMX \\
        & & \textbf{Reformulated:} \textcolor{red}{RuntimeMXBean} Determine Java version through JMX \\
        \midrule
        \multirow{2}*{SEQUER} & \multirow{2}*{expansion} & \textbf{Original:} Java reverse string \\
        & & \textbf{Reformulated:} Java reverse string \textcolor{red}{to reverse} \\
        \midrule
        \multirow{2}*{NLPAUG - SO word2vec} & \multirow{2}*{expansion} & \textbf{Original:} Convert from Radians to Degrees in Java  \\
        & & \textbf{Reformulated:} Convert from \textcolor{red}{AV} Radians to Degrees in \textcolor{red}{Long} Java \\
        \midrule
        \multirow{2}*{NLPAUG - BERTOverflow} & \multirow{2}*{expansion} & \textbf{Original:} Java reverse string \\
        & & \textbf{Reformulated:} java reverse \textcolor{red}{character} string \\
        \midrule
        \multirow{2}*{NLPAUG - Google News Word2vec} & \multirow{2}*{expansion} & \textbf{Original:} Constructs a new synchronized Set based on a HashSet \\
        & & \textbf{Reformulated:} \textcolor{red}{PROTEGE} Constructs a new synchronized Set \textcolor{red}{BUT} based on \textcolor{red}{lend} a HashSet \\
        \midrule
        \multirow{2}*{Google Prediction Service} & \multirow{2}*{modification} & \textbf{Original:} Copying from an Input Stream to a File \\
        & & \textbf{Reformulated:} \textcolor{red}{\sout{Copying}} copy \textcolor{red}{\sout{from an}} inputstream to \textcolor{red}{\sout{a}} file \\
    \midrule
        \multirow{3}*{NLPAUG - SO Word2vec} & \multirow{3}*{modification} & \textbf{Original:} get value from private field having object ``Field". JAVA \\
        & & \tabincell{l}{\textbf{Reformulated:} get \textcolor{red}{\#\#.\#\#\#mlrd\_rbl sent \sout{value from}} private field having object \\ ``\textcolor{red}{Tennis\_Complex \sout{Field}} ". JAVA} \\
        \midrule
        \multirow{2}*{NLPAUG - Google News Word2vec} & \multirow{2}*{modification} & \textbf{Original:} How to extract a string between two delimiters\\
        & & \textbf{Reformulated:} How to extract a string between \textcolor{red}{Three curly\_braces \sout{two delimiters}} \\
        \midrule
        \multirow{2}*{NLPAUG - BERTOverflow} & \multirow{2}*{modification} & \textbf{Original:} How do I calculate difference between two dates \\
        & & \textbf{Reformulated:} how do \textcolor{red}{they \sout{I}} calculate \textcolor{red}{months \sout{difference}} between two dates \\
        \midrule
        \multirow{2}*{NLPAUG - WordNet} & \multirow{2}*{modification} & \textbf{Original:} How can I cast a Long to an int in Java \\
        & & \textbf{Reformulated:} How \textcolor{red}{hindquarters Unity \sout{can I}} cast a Long to an int in \textcolor{red}{Coffee \sout{Java}} \\
        \midrule
        \multirow{2}*{NLPAUG - Random} & \multirow{2}*{modification} & \textbf{Original:} BigDecimal greater than Zero \\
        & & \textbf{Reformulated:} BigDecimal \textcolor{red}{less \sout{greater}} than Zero \\
    \midrule
        \multirow{2}*{NLPAUG - Random} & \multirow{2}*{deletion} & \textbf{Original:} Get min value between two double type value \\
        & & \textbf{Reformulated:} Get min value between two \textcolor{red}{\sout{double type}} value \\
    \bottomrule
    \end{tabular}
    \label{tab:reformex}
\end{table*}
